Addressing memory bandwidth scalability in vector processors for streaming applications

As the size of artificial intelligence and machine learning (AI/ML) models and datasets grows, the memory bandwidth becomes a critical bottleneck. The paper presents a novel extended memory hierarchy that addresses some major memory bandwidth challenges in data-parallel AI/ML applications. While data-parallel architectures like GPUs and neural network accelerators have improved power performance compared to traditional CPUs, they can still be significantly bottlenecked by their memory bandwidth, especially when the data reuse in the loop kernels is limited. Systolic arrays (SAs) and GPUs attempt to mitigate the memory bandwidth bottleneck but can still become memory bandwidth throttled when the amount of data reuse is not sufficient to confine data access mostly to the local memories near to the processing. To mitigate this, the proposed architecture introduces three levels of on-chip memory -- local, intermediate, and global -- with an ultra-wide register and data-shufflers to improve versatility and adaptivity to varying data-parallel applications. The paper explains the innovations at a conceptual level and presents a detailed description of the architecture innovations. We also map a representative data-parallel application, like a convolutional neural network (CNN), to the proposed architecture and quantify the benefits vis-a-vis GPUs and repersentative accelerators based on systolic arrays and vector processors.

==> parts/innovations.tex <==
\section{Architectural Innovations}\label{sec:decisions}
In this section, we present the key architectural innovations that address the memory bandwidth and the utilization
challenges faced by architectures targetting data-parallel applications, specifically ML/AI applications. 


In the proposed architecture, several processing tiles are combined into a chip-wide processing platform. Here we focus only on a single tile. Inside each tile, there are three levels of on-chip data buffers: local, intermediate, and global. While
such three levels of memory hierarchy are not uncommon, the key differentiation and innovation is the ultra-large width
of the intermediate and global data buffers and the use of 2 specialized data-shufflers which work complementary, in order  to make it more versatile and adaptive to the
varying needs of data-parallel applications. This is conceptually shown in Figure~\ref{fig:provet_hierarchy}. 

We note that we avoid the usage of the term \emph{memory} and instead call these \emph{data buffers} as this better
describes how these storage elements are used and designed.

We now briefly discuss the three levels of data buffers and the connection between them starting from the lowest level,
and later motivate the rationale of the choices.\bigskip

The local data buffers are small and tightly integrated with Vector Functional Units (VFUs), and their width is matched
with the VFUs. Basically, they are realized as two-port register units. Their purpose is to hold constants and intermediate variables generated during computation to minimize the
relatively expensive access to the intermediate and global memory components. The number of VFUs along with its local
memory is a design time decision and decides the degree of data parallelism.

The intermediate-level data buffer component is a limited set of very wide stack of single-port register cells (VWRs) that are
asymmetric in their interface: on one side its interface width is matched to that of the global memory assigned to the tile, and on the other
side its width is matched to that of VFUs. 

The global tile memory is as wide as the VWR and holds the bulk of the data used in data-parallel applications.

Between the three elements two specialized shufflers, one fine-grained and the other coarse-grained, allow rearranging of the data when it
moves between the different memory hierarchy levels.\bigskip

The ability of the memory hierarchy proposed above to address the challenges of energy-efficient memory access and
utilization are predicated on the following insights:

\subsection{Ultra-wide shallow memory}\label{sec:ultra_wide_mem}
Reading data from an ultra-wide memory is more energy efficient compared to reading multiple times for a significantly
narrower memory. Upon inspecting the internal structure of a SRAM it is easy to observe that scaling the width or the
depth has very different costs. To illustrate this in a qualitative way with a 
parameterized model, we start with an example of a WxD SRAM (width x depth) as shown in
Figure~\ref{fig:sram_structure}. 

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.7\linewidth]{img/sram_structure.pdf}
    \caption{Simplified internal SRAM structure}
    \label{fig:sram_structure}
\end{figure}

% \begin{figure}[b]
%   \begin{subfigure}[b]{0.44\linewidth}
%     \centering
%     \includegraphics[width=0.8\linewidth]{img/square_cells.pdf}
%     \caption{Arrangement with aspect ratio = 1}
%     \label{fig:square_cells}
%   \end{subfigure}\hfill%
%   \begin{subfigure}[b]{0.55\linewidth}
%     \centering
%     \includegraphics[width=0.8\linewidth]{img/flat_cells.pdf}
%     \caption{Arrangement with aspect ratio \~1}
%     \label{fig:flat_cells}
%   \end{subfigure}%
%   \todo[inline]{align bottom of the image}
%   \caption{Different possible arrangements for multiple memory cells showing the
%   conceptual length of reading from a cell}
%   \label{fig:cell_arrangement}
% \end{figure}

If we now analyse the costs of fetching a row of data, we now need to energize $W$ bit lines ($BL$) and 1-word line
($WL$). Let us assume that the cost of energizing bit and word lines is proportional to its length. %For this data
operation, the cost of energizing the bit and word lines can be written as: 

% \begin{equation}
%     \overbrace{W \cdot D \cdot BL}^{\text{energize}\ W\ \text{bitlines}} + \underbrace{1 \cdot W \cdot WL}_{{\text{energize}\ 1\ \text{wordline}}}
%     \label{eq:cost_per_word}
% \end{equation}

Where W is the width of the SRAM, D is the depth, DL and WL is the cost of energizing a bit/word line segment of size 1.  

%If we now compute of energizing the bit and word lines, normalized for the amount of data we are reading we obtain: 

% \begin{equation}
% \label{eq:cost_per_bit}
% \frac{W \cdot D \cdot BL + 1 \cdot W \cdot WL}{W} = D\cdot BL + WL
% \end{equation}


%\todo[inline]{address why it is not done today (wide memory)}

It now becomes clear that increasing the width of the SRAM does not impose a penalty in the normalized cost of
energizing the wires (within the assumptions of this simplified model) however, increasing the depth will severely
penalise large memories.

To quantify this with actual numbers, we show the simulated normalized energy reported by CACTI simulator \cite{6386626} for a fixed size
memory of 64 Kbit but sweeping its I/O port size from 64 to 4 Kbit. The results are shown in
Figure~\ref{fig:memory_cost}.

%\begin{figure}[b]
%    \centering
%    \includegraphics[width=0.6\linewidth]{img/energy_scaling.png}
%    \caption{Total energy cost reported by CACTI for a memory array of total size 64 Kbit varying the size of the port. The energy is normalized for each bit that is written/read}
%    \label{fig:memory_cost}
%\end{figure}

\begin{figure}[b]
\centering
\begin{tikzpicture}
\begin{axis}[
    %title={Total energy per bit},
    xlabel={Bus width (bits)},
    ylabel={Energy (pJ)},
    grid=none,
    width=0.6\textwidth,
    height=0.4\textwidth,
    xtick={0,2048,...,8192},
    minor x tick num=4,
    tick pos=left,
]
\addplot table [x=bus_width, y=energy_per_bit, col sep=comma, mark=none] {data/energy_vs_width.csv};
\end{axis}
\end{tikzpicture}
\caption{The relationship between bus width and energy per bit.}
\label{fig:memory_cost}
\end{figure}

The main takeaway from Figure~\ref{fig:memory_cost} is that the width scaling reduces the energy per bit. There is,
however, a big assumption that needs to hold true, the movement of data needs to be predominantly in the vertical
direction along the bits. This means that the data that is positioned on the left side of the memory needs to be consumed by the
processing elements that are aligned with the left side of the memory as well. If this assumption does not hold true,
all the gains from increasing the width can potentially be lost in the increased cost of moving the data horizontally opposite to the bits.
This does not mean that horizontal data movement should never occur, however, vertical movement needs to be predominant
for this arrangement of the memory to provide benefits. Fortunately, we have observed in mapping experiments (see mapping section?) that this assumption is valid in our target application domain.

Increasing the width of the memory is not only concerning the physical length of the word lines but also how the
multiple memory cells are arranged in the \emph{block-level} floorplan. To access a memory cell it is necessary to cross
a number of other cells in the square arrangement. However, there is no crossing for the shallow-wide arrangement. On
average, an array with $N$ cells that is arranged in a square it will be necessary to cross $\sqrt{N}/2$ cells, but on
the flat arrangement it will never have to cross any cell. It is important to clarify that the above assumes that the
\emph{horizontal} movement of data can be considered as negligible.  The way this is achieved in our novel proposal is
clarified in section \ref{sec:detailed_description}.

\subsection{Memory asymetry}\label{sec:memory_assymetry}
Reading and writing between VWR from VFU is more energy efficient compared to that between VFU and the main memory.
Further, since the VFU width is 10X to 100X less than that of VWR, once a data has been loaded into the VWR, the VFU can avoid going
to the main memory 10X to 100X times.  This ratio is further amplified if one considers the exploitation of the data
locality. However, and that is unique to our proposal, even for low data locality and
data reuse factors, this asymetric interface still significantly alleviates the memory bottleneck, as just explained!

Note that the SA architectures have the same objective of avoiding expensive access to the main memory by directly
feeding the output of one PE into another. However, as pointed before, SAs work well as long as the data flow of an
application is a good match to the dimensions of the SA. If there is a mismatch, the utilization will quickly degrade. 

The memory hierarchy in our proposed solution substantially mitigates the memory bottleneck issue to a greater extent
than what traditional systolic array architectures can offer. Systolic arrays largely depend on potential local data
reuse to reduce the number and frequency of global memory accesses. However, whenever new data is demanded for
computation, it necessitates fetching from the global memory, thereby introducing latency.

Contrarily, our proposed solution capitalizes on the asymmetry of the data ports to diminish the frequency of SRAM
access. This approach does not solely rely on data reuse opportunities for minimizing memory access. Instead, it employs
an intelligent memory management strategy that leverages the asymmetric nature of data ports, thereby reducing the need
for frequent main memory accesses. Hence, the mapping methodology has to be adapted to enable this feature (see mapping section again?).

% the following paragraph looks redundant and I doubt that it helps
Upon integrating data reuse opportunities into this methodology, the frequency of main memory accesses reduces even
further. This combined strategy of exploiting data port asymmetry and data reuse effectively minimizes memory access
requirements, thereby addressing the persistent memory bottleneck problem more effectively than traditional systolic
arrays.

\subsection{Data rearangement} \label{sec:data_rearrangement}
Two shufflers which act in a fully complementary way are present: one between main memory and the VWRs, and the other integrated in the VFUs. These shufflers
contribute to making the memory hierarchy fully adaptive to the varying dataflows of the data-parallel applications.
This ensures that the VFUs and the memory channels have a high-level utilization for different.

Since the VFU and VWRs are pitch matched, a given VFU can only access the data that is placed in the region of the VWR
that is aligned with itself. To enable access to other regions of the VWR we propose a coarse-grained shuffler (tile shuffler) between
the VWR and SRAM. This shuffler can be used to move data when it is loaded into the VWR and also once the data is
already in the VWR. By using this shuffler, the data can be prepared so that the VFU that requires it will be able to
access it when needed. The fine-grained shuffler inside the VFUs acts similar to a traditional data shuffler used for vector processors [add ref].
An illustrative example on how the shufflers are used is provided in section \ref{sec:example}.

Shufflers serve an analogous function to the PE interconnect network of a systolic array. They distribute the data to
the location where the computation elements require it. However, the advantage of the shufflers over the normal SA interconnect
networks is that they can span larger distances more efficiently. In SA architectures, data can only move from one PE to
its nearest neighbor. Instead, using a shuffler, data can potentially even go from one end of the data word to the other
in a single step. This effect is more pronounced as the size of the architecture increases. However, in practice, by applying a careful mapping approach, we avoid having to go to move further than a small window around each PE slot. Thus it is only
rarely that we have to activate the more energy-consuming longer shuffler sections in our logarithmic shuffler
component. Still, having that functionality is essential for our competitive advantage compared to the SA alternatives.

\subsection{Data organization} \label{sec:data_organization} The above arguments assume that the data in the main memory
is available in an application-specific way to enable their exploitation by a specific data flow, i.e.\ the data layout
is compatible with the particular architecture instance and the mapping.  This is a one-time effort, and a library of
such organization patterns can be created to amortize the engineering cost. The library development falls out of the
scope of this paper but an example is provided for a convolution layer in section \ref{sec:example}. This library-based
approach is analogous to the libraries commonly used in the development of ML applications, such as PyTorch or
Tensorflow, among others. So it does not incur a disadvantage for our approach.

These arguments will be made more concrete in section~\ref{sec:example} when we map a CNN to a specific instance of the
proposed architectural template that is described in detail in the next section.



==> parts/sota.tex <==
\section{State of the art review and comparison\label{sec:state_of_the_art}}
The proposed architecture might have similarities with other well-known architectures that have been present in the
community for several years. To clarify and distinguish the similarities and key differences to other architectures, a
set of them is listed in this section. A brief description of the main characteristics is shown as well as the key
differences to the proposed architecture.

\subsection{Eyeriss}
The Eyeriss accelerator is a Ml/AI accelerator based on a systolic array structure. However the Eyeriss processing
elements include a small local memory that allows to exploit the reuse of data within one PE. This also allows to
directly implement convolutions without relying on the img2col transformation. However Eyeriss uses a 2D organization
for the PE structure which, as explained in \ref{sec:motivations} and \ref{sec:ultra_wide_mem}, introduces scalability
problems that prevent expanding the size of the array beyond a limited size.
\subsection{TPU}
The Edge TPU is a system-on-chip (SoC) that includes a tensor processing unit, a general-purpose CPU, and various memory
and I/O interfaces. The tensor processing unit is optimized for the efficient execution of convolutional neural networks
(CNNs) and other types of deep learning models, using a matrix multiplication engine and hardware accelerators for
common operations such as pooling, activation, and quantization. The Edge TPU also includes a software stack that
provides APIs for model deployment, inference, and management, as well as support for popular machine learning
frameworks such as TensorFlow and PyTorch.

Since Edge TPU is based on a matrix multiplication engine, it depends on the usage of the img2col transformation. As has
been explained in previous sections this approach introduces data redundancy and overhead in performing the
transformation. 

The two main differences between the proposed architecture are the use of 1D organization of the memory and compute
resources (explained in \ref{sec:ultra_wide_mem}) and the direct implementation of convolution instead of relying in
img2col (explained in \ref{sec:example}).
\subsection{ARA (Adaptive RISC-V Architecture)}
The ARA (Adaptive RISC-V Architecture) is a configurable and scalable 64-bit RISC-V vector processor developed by the
PULP  research group that utilizes the RISC-V vector extension (RVV). ARA features a multi-lane architecture, where each
lane can execute a vector instruction independently. This architecture incorporates one wide memory for each lane,
similar how Provet uses a wide memory for each VFU. However, each lane in ARA has a separate memory and thus sharing of
data between lanes requires a comple interconnect infrastructure. In contrast, Provet uses a single memory that is
shared between all the VFUs. This allows for a much simpler interconnect infrastructure (shuffler) that can be used to
share data between VFUs. 

The benefits obtained in terms of PE utilization in Provet are also present in ARA given that the wide memory provides a
large bandwidth that does not bottleneck the PEs. However, the different implementation of the memory hierarchy in ARA
makes it difficult to scale the architecture to larger sizes and its energy efficiency does not scale as well as Provet
when increasing the number of lanes, due to the fact that each lane utilizes a new memory, with its own energy overhead.
However, given the focus of this paper in utilization and memory bandwidth, a more detailed comparison of the energy
efficiency of both architectures is left for future work.


